Why Stop at Software? Recursive Self-Improvement Reaches Robot Hardware

Agentic robots can improve their control programs and manipulation skills through experience, yet the hardware through which they act and sense typically remains fixed. We introduce HardwareRSI, to our knowledge the first framework for recursive self-improvement (RSI) of robot hardware in which a closed-loop manipulation agent can redesign its own hardware, including its mechanisms and sensors. The agent identifies limitations of its current hardware from execution feedback and uses observations from each modified design to guide the next hardware change. We further develop HardwareRSI-Bench to evaluate RSI of robot hardware across eight classes of simulated manipulation tasks drawn from real jobs. Within a budget of 30 attempts per task, the agent completes 33 of 36 tasks. It completes 3 with its original hardware and 30 after redesign, with multiple hardware changes on 21 of those 30 tasks. To test whether one hardware design can serve a family of related tasks, we evaluate four families of three tasks each. In three of these families, the agent solves all three tasks with the same design. A single design also completes a four-stage assembly task spanning multiple classes. The agent keeps improving after its first success: more efficient designs and practice cut the control steps a task takes by a median of 22%. On a physical robot, the agent uses feedback from a failed box lift to design gripper sleeves and successfully lifts the box with them.

==> sections/teaser.tex <==
\makeatletter
\let\psi@titleblock\@maketitle
\renewcommand{\@maketitle}{\psi@titleblock
  \begin{center}
  \includegraphics[width=\textwidth]{figures/fig1_5p.pdf}
  \end{center}
  \vspace{-0.6em}
  \setcounter{figure}{0}%
  \captionof{figure}{\textbf{\sysname{} for recursive self-improvement (RSI) of robot hardware.}
\textbf{(a)} An agent that revises its control software still acts and senses through the same hardware. In \sysname{}, the agent can also edit the hardware design in CAD, operate the modified robot, and use the resulting observations to guide its next redesign.
\textbf{(b)} In simulation, the original gripper is too wide to enter the bin (v0). A suction cup on a long rod reaches the bracket, but the bin rim obscures the contact (v1). Repositioning the wrist camera reveals that the bracket's flat face is too narrow for the cup to seal (v2). The agent switches to long fingers (v3) and, after the bracket slips, adds rubber tips that allow it to lift the bracket out (v4). The insets show the wrist-camera views before and after repositioning. Labels above each trial show the hardware configuration, and labels below give the outcome. Agent-designed parts are orange, with earlier additions in lighter shades. The bracket is blue.
\textbf{(c)} On a physical arm, the original gripper grasps only a corner of a wide box, and the box slips. The agent designs sleeves that fit over the gripper fingers (CAD model in inset) and lifts the box with the printed sleeves. After the first successful lift, the agent continues the recursive self-improvement loop with the redesigned gripper, reducing the lift time from 15.6\,s to 9.0\,s.}
  \label{fig:teaser}
  \vspace{0.2em}}
\makeatother

